Concurrency and Probability: Removing Confusion, Compositionally

Assigning a satisfactory truly concurrent semantics to Petri nets with confusion and distributed decisions is a long standing problem, especially if one wants to resolve decisions by drawing from some probability distribution. Here we propose a general solution based on a recursive, static decomposition of (occurrence) nets in loci of decision, called structural branching cells (s-cells). Each s-cell exposes a set of alternatives, called transactions. Our solution transforms a given Petri net into another net whose transitions are the transactions of the s-cells and whose places are those of the original net, with some auxiliary structure for bookkeeping. The resulting net is confusion-free, and thus conflicting alternatives can be equipped with probabilistic choices, while nonintersecting alternatives are purely concurrent and their probability distributions are independent. The validity of the construction is witnessed by a tight correspondence with the recursively stopped configurations of Abbes and Benveniste. Some advantages of our approach are that: i) s-cells are defined statically and locally in a compositional way; ii) our resulting nets faithfully account for concurrency.

==> abstract.tex <==
% !TEX root =  main.tex

\begin{abstract}
Assigning a satisfactory truly concurrent semantics to Petri nets with confusion and distributed decisions is a long standing problem, especially if one wants to resolve decisions by drawing from some probability distribution.
%
Here we propose a general solution based on a recursive, static decomposition of (occurrence) nets in loci of decision, called \emph{structural branching cells} (\emph{s-cells}). 
Each s-cell exposes a set of alternatives, called \emph{transactions}.
%
Our solution  transforms  a given Petri net into another net whose transitions are the transactions of the s-cells and whose places are those of the original net, with some auxiliary structure for bookkeeping. The resulting net is confusion-free, 
and thus conflicting alternatives can be equipped with probabilistic choices, while nonintersecting alternatives are purely concurrent and their probability distributions are independent.
%
The validity of the construction is witnessed by a tight correspondence with the recursively stopped configurations of Abbes and Benveniste.  
Some advantages of our approach are that: 
i)~s-cells are defined statically and locally in a compositional way;
ii)~our resulting nets faithfully account for concurrency.%exhibit the complete concurrency property.
\end{abstract}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main.tex"
%%% End:


==> taste.tex <==
% !TEX root =  main.tex
%\vspace{-5pt}

\begin{figure}[t]
\begin{subfigure}[b]{0.25\textwidth} 
$$
 \xymatrix@R=1.2pc@C=.6pc{
 \drawmarkedplace\ar[d]\ar[rrd]
  \nameplaceup 1
 &
 \drawpersistentplace\ar@[mygray][d]
 \namepersup 1
 \\
 \drawtrans a\ar[d]\ar@[mygray][rd]
 & \drawtransu {}\ar@[mygray][d]\ar@[mygray][rd] 
 & \drawtrans d\ar@[mygray][d]\ar[rd]
 \\
 \drawplace
 \nameplaceright 3 
 &
 \drawpersistentplace
 \namepersright 6
 &
 \drawpersistentplace
 \namepersright 3 
 &
 \drawplace
 \nameplaceright 6 
 }
$$
\subcaption{S-cell $\bc_1$}\label{fig:taste1}
\end{subfigure}
\hspace{2cm}
\begin{subfigure}[b]{0.35\textwidth} 
$$
 \xymatrix@R=1.2pc@C=.9pc{
 \drawpersistentplace \ar@[mygray][d] 
 \namepersup 2
 &
 \drawpersistentplace \ar@[mygray][d]
 \namepersup 3 
 &&
 \drawmarkedplace \ar@{-->}[ld]\ar[d]\ar[rd]
 \nameplaceup 2
 &
 \drawplace \ar[ld]\ar[d]
 \nameplaceup 3
 \\
 \drawtransu {}\ar@[mygray][rd]\ar@[mygray]@(dr,ul)[rrrrd]
 & \drawtransu {}\ar@[mygray][d]\ar@[mygray][r] 
 & \drawtransd b\ar@{-->}[d]
 & \drawtrans b\ar@[mygray][lld]\ar[ld]
 & \drawtrans c\ar@[mygray][d]\ar[ld]
 \\
 &
 \drawpersistentplace
 \namepersright 5
  &
 \drawplace
 \nameplaceright 4
 &
 \drawplace
 \nameplaceright 5
 &
 \drawpersistentplace
 \namepersright 4
  &
 &
 &
 }
$$
\subcaption{S-cell $\bc_2$ and its sub s-cell $\bc_3$}\label{fig:taste2}
\end{subfigure}
\par
\begin{subfigure}[b]{0.32\textwidth} 
$$
 \xymatrix@R=.8pc@C=.6pc{
 &
 &
 \drawmarkedplace \ar[ld]\ar[rd]
 \nameplaceright 1 
 \\
 &
 \drawtrans d\ar@[mygray][dl]\ar[d]
 && \drawtrans a\ar@[mygray][dl]\ar[rd]
 \\
 \drawpersistentplace \ar@[mygray][d]
 \namepersright 3
 &
 \drawplace 
 \nameplaceright 6
 &
 \drawpersistentplace 
 \namepersup 6
 &
 \drawmarkedplace \ar[ld]\ar[d]\ar[rd]
 \nameplaceup 2
 &
 \drawplace \ar[ld]\ar[d]
 \nameplaceup 3
 \\
 \drawtransu {}\ar@[mygray][d]\ar@[mygray][r] 
 &
 \drawpersistentplace \ar@[mygray][r]
 \nameplaceup {\color{mygray}p_b}
 & \drawtransu b\ar[d]
 & \drawtrans b\ar@[mygray]@(dl,ur)[llld]\ar[ld]
 & \drawtrans c\ar@[mygray][d]\ar[ld]
 \\
 \drawpersistentplace
 \namepersright 5
 &&
 \drawplace
 \nameplaceright 4
 &
 \drawplace
 \nameplaceright 5
 &
 \drawpersistentplace
 \namepersright 4
 }
$$
\subcaption{Flat net (pruned)}\label{fig:taste3}
\end{subfigure}
%\caption{Structural cells as dynamic nets and their composed, flattened version}\label{fig:taste}
%\end{figure}
%\begin{figure}[t]
\begin{subfigure}[b]{0.17\textwidth} 
$$
 \xymatrix@R=.8pc@C=.3pc{
 &&
 \drawmarkedplace \ar[rd]
 \nameplaceright 1
 \\
 {\phantom{d}} &&& \drawtrans a\ar@[mygray][dl]\ar[rd]
 \\
 &
 &
 \drawpersistentplace 
  \namepersup 6
 &
 \drawmarkedplace \ar[d]
 \nameplaceup 2
 &
 \drawplace \ar[ld]
 \nameplaceup 3
 \\
 &
 & 
 & \drawtrans b\ar@[mygray]@(l,ur)[llld]\ar[ld]
 & 
 \\
 \drawpersistentplace
 \namepersright 5 &&
 \drawplace
 \nameplaceright 4
 &
 &
 }
$$
\subcaption{$a\preceq b$}\label{fig:tasteproc1}
\end{subfigure}
\begin{subfigure}[b]{0.20\textwidth} 
$$
\xymatrix@R=.8pc@C=.3pc{
 \drawmarkedplace \ar[rd]
 \nameplaceright 1
 \\
  {\phantom{d}} & \drawtrans a\ar@[mygray][dl]\ar[rd]
 \\
 \drawpersistentplace 
 \namepersup 6
 &
 \drawmarkedplace \ar[rd]
 \nameplaceup 2
 &
 \drawplace \ar[d]
 \nameplaceup 3
 \\
  {\phantom{b}} && 
 \drawtrans c\ar@[mygray][d]\ar[ld]
 \\
 &
 \drawplace
 \nameplaceright 5
 &
 \drawpersistentplace
 \namepersright 4
 }
$$
\subcaption{ $a\preceq c$}\label{fig:tasteproc2}
\end{subfigure}
\begin{subfigure}[b]{0.15\textwidth} 
$$
 \xymatrix@R=.8pc@C=.3pc{
 &
 &
 \drawmarkedplace \ar[ld]
 \nameplaceright 1
 \\
 &
 \drawtrans d\ar@[mygray][dl]\ar[d]
 \\
 \drawpersistentplace \ar@[mygray][d]
 \namepersright 3
 &
 \drawplace 
 \nameplaceright 6
 &
 &
 \drawmarkedplace \ar[ld]
 \nameplaceup 2
 \\
 \drawtransu {}\ar@[mygray][d]\ar@[mygray][r] 
 &
 \drawpersistentplace \ar@[mygray][r]
 \nameplaceup{\color{mygray}p_b}
 & \drawtrans b\ar[d]
 \\
 \drawpersistentplace
 \namepersright 5
 &&
 \drawplace
 \nameplaceright 4
 }
$$
\subcaption{ $d\preceq b$}\label{fig:tasteproc3}
\end{subfigure}
\caption{S-cells, confusion-free p-net and processes for the net in Fig.~\ref{fig:condconfusion}}\label{fig:tasteproc}
\end{figure}

%\input{figura-hernan}

\paragraph{A Taste of the Approach.}

We sketch the main ideas over the net in Fig.~\ref{fig:condconfusion}.
%AB's branching cells are defined dynamically
%%, as the computation progresses
%(see Fig.~\ref{fig:AB1}): initially there is a choice between $a$ and $d$. 
%If $a$ is chosen, 
%then $d$ disappears 
%%from the event structure, 
%leading to a second cell with a choice between $b$ and $c$. 
%If instead $d$ is chosen, then $a$ and $c$ disappear, 
%leading to a third cell whose only option is $b$. 
%Thus, the reachable maximal configurations t
%%hat can be reached 
%are 
%$\{a,b\}$ (with no dependency), 
%$\{a \preceq c\}$ and 
%$\{b,d\}$ (with no dependency). 
%For example, the  sequence $\sigma=b a$ is legal w.r.t. $\{a,b\}$ but not executable.
%
%The structural branching cell decomposition that we propose operates on the net and is done statically.
%In our approach, s-cells are defined statically.
In our approach, there are two main s-cells: $\bc_1$ associated with $\{a,d\}$, and $\bc_2$ with $\{b,c\}$.
There is also a nested s-cell $\bc_3$ with $\{b\}$ that arises from the decomposition of the subnet $\remInitial {N_{\bc_2}} 3$.
S-cells are shown in Fig.~\ref{fig:scellscondconfusion}.
Their dynamic nets are in Figs.~\ref{fig:taste1}--\ref{fig:taste2},
where auxiliary transitions are in grey and unlabeled. Places $\mathbf{\overline{1}}$ and $\mathbf{\overline{2}}$
(and their transitions) are irrelevant, because the places $1$ and $2$ are already marked. 
However, our cells being static, we need to introduce auxiliary places in all cases.
Note that in Fig.~\ref{fig:taste2} there is an arc between two transitions.
This is because the target transition is dynamically created when the other is executed (hence the dashed border).
Also note that there are two transitions with the same label $b$: one is associated with the s-cell $\bc_2$, the other with the unique s-cell of $\remInitial {N_{\bc_2}} 3$ and is released when the place $\mathbf{\overline{3}}$ becomes marked.

After the s-cells are assembled and flattened we get the p-net in Fig.~\ref{fig:taste3} (where irrelevant nodes are pruned).
%
Initially, only $a$ and $d$ are enabled. If $a$ is fired, we reach the marking $\{2,3,\mathbf{\overline{6}}\}$ where $b:\{2,3\}\to \{4,\mathbf{\overline{5}}\}$ and $c:\{2,3\}\to \{\mathbf{\overline{4}},5\}$ are enabled (and in conflict). 
If $d$ is fired, we reach the marking $\{2,\mathbf{\overline{3}},6\}$ where only the auxiliary transition can be fired, 
%leading to $\{2,\mathbf{\overline{3}},\mathbf{\overline{5}},6,\mathbf{p}_b\}$ and 
enabling $b:\{2,\mathbf{p}_b\} \to 4$. The net is confusion-free, as every conflict involves transitions with the same preset. For example, as the places $3$ and $\mathbf{\overline{3}}$ (and thus $\mathbf{\overline{p}}_b$) are never marked in a same run,
the transitions $b:\{2,3\}\to \{4,\mathbf{\overline{5}}\}$ and $b:\{2,\mathbf{p}_b\} \to 4$ will never compete for the token in $2$.

Last, Figs.~\ref{fig:tasteproc1}--\ref{fig:tasteproc3} show the  maximal processes of the net in Fig.~\ref{fig:taste3}.
%that represent the possible executions of the net.
%We note that, as expected, no concurrent execution are allowed, because the choice between $a$ and $d$ drives the decision in the other cells. 
It is evident that $b$ can be executed neither before $a$ nor before $d$ (and the trace $b;a$ is not legal and not executable).
%A more sophisticated example of a process with causal OR-dependencies is shown in Section~\ref{sec:concurrency}.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main.tex"
%%% End:

